Comprehensive Monitor-Oriented Compensation Programming

Compensation programming is typically used in the programming of web service compositions whose correct implementation is crucial due to their handling of security-critical activities such as financial transactions. While traditional exception handling depends on the state of the system at the moment of failure, compensation programming is significantly more challenging and dynamic because it is dependent on the runtime execution flow - with the history of behaviour of the system at the moment of failure affecting how to apply compensation. To address this dynamic element, we propose the use of runtime monitors to facilitate compensation programming, with monitors enabling the modeller to be able to implicitly reason in terms of the runtime control flow, thus separating the concerns of system building and compensation modelling. Our approach is instantiated into an architecture and shown to be applicable to a case study.

==> eptcsdata.tex <==
\providecommand{\firstpage}{47}
\providecommand{\publicationstatus}{B. Buhnova, L. Happe, J. Kofro\v n (Eds.): Formal Engineering\\
Approaches to Software Components and Architectures 2014\\
EPTCS 147, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.147.4}{10.4204/EPTCS.147.4}}
\pdfoutput=1

